Reconfigurable Inverted Index

Existing approximate nearest neighbor search systems suffer from two fundamental problems that are of practical importance but have not received sufficient attention from the research community. First, although existing systems perform well for the whole database, it is difficult to run a search over a subset of the database. Second, there has been no discussion concerning the performance decrement after many items have been newly added to a system. We develop a reconfigurable inverted index (Rii) to resolve these two issues. Based on the standard IVFADC system, we design a data layout such that items are stored linearly. This enables us to efficiently run a subset search by switching the search method to a linear PQ scan if the size of a subset is small. Owing to the linear layout, the data structure can be dynamically adjusted after new items are added, maintaining the fast speed of the system. Extensive comparisons show that Rii achieves a comparable performance with state-of-the art systems such as Faiss.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	mm18.tex


PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF} compress

# Added by Y. Matsui
compress: mm18.pdf
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=output.pdf mm18.pdf
	#gs -o output.pdf -dNoOutputFonts -sDEVICE=pdfwrite mm18.pdf  # Converts all texts to vector lines
	rm mm18.pdf
	mv output.pdf mm18.pdf



%.pdf:  %.dtx   $(PACKAGE).cls
#	pdflatex $<
	pdflatex -shell-escape $<
	- bibtex $*
#	pdflatex $<
	pdflatex -shell-escape $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
#	pdflatex $<
	pdflatex -shell-escape $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -shell-escape $<; done
#	do pdflatex $<; done


%.cls:   %.ins %.dtx
#	pdflatex $<
	pdflatex -shell-escape $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
#	pdflatex $<
	pdflatex -shell-escape $<
	- bibtex $*
#	pdflatex $<
	pdflatex -shell-escape $<
#	pdflatex $<
	pdflatex -shell-escape $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -shell-escape $<; done
#	do pdflatex $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


# clean:
# 	$(RM)  $(PACKAGE).cls *.log *.aux \
# 	*.cfg *.glo *.idx *.toc \
# 	*.ilg *.ind *.out *.lof \
# 	*.lot *.bbl *.blg *.gls *.cut *.hd \
# 	*.dvi *.ps *.thm *.tgz *.zip *.rpi


clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst

